PerturbGS: Fast and Scalable Gaussian Splatting via Camera Perturbations

Fast and scalable 3D Gaussian Splatting (3DGS) reconstruction from unposed input views requires both computational efficiency and geometric reliability. With dense views, Structure-from-Motion (SfM) preprocessing dominates the total reconstruction time, and initializing Gaussians from the pixel-wise predictions of a 3D vision foundation model (3D-VFM) can exhaust GPU memory. With sparse views, wide baselines can cause SfM registration to fail, and pose and depth errors in the predictions of the 3D-VFM can introduce artifacts in novel views. We propose PerturbGS, a view-count-agnostic framework for fast and scalable 3DGS reconstruction from both dense and sparse views. Our key insight is to use camera perturbations to expose geometric ambiguity before and during 3DGS training. Before 3DGS training, our Camera-Perturbation-based Initialization (CPI) identifies depth-inconsistent point clouds through camera perturbations and removes them along with duplicate point clouds, yielding a compact initialization for 3DGS training. During 3DGS training, our Camera-Perturbation-based Adaptive density control (CPA) prunes Gaussians with low rendering contribution across input and perturbed views. Through camera perturbations, our CPA also groups Gaussians and densifies them group-wise, which limits the redundant growth of Gaussians. Our PerturbGS reconstructs 3D scenes from dense views where previous methods exhaust GPU memory and produces sharper novel views with reduced artifacts from sparse views.

==> arXiv/cmlab_preamble.tex <==
\RequirePackage{iftex}
\ifPDFTeX\else
  \newcount\pdfcompresslevel
  \newcount\pdfoptionpdfminorversion
  \newcount\pdfgentounicode
  \providecommand{\pdfcatalog}[1]{}
  \providecommand{\pdfglyphtounicode}[2]{}
\fi

\usepackage{xcolor}
\definecolor{cmlabPrefix}{HTML}{0D207F}  %
\definecolor{cmlabNumber}{HTML}{0D207F}  %
\definecolor{cmlabCite}{HTML}{0D207F}    %
\definecolor{cmlabURL}{HTML}{0D207F}     %

\usepackage{hyperref}
\hypersetup{
  colorlinks=true,
  linkcolor=cmlabNumber,    %
  citecolor=cmlabCite,      %
  urlcolor=cmlabURL,        %
  filecolor=cmlabURL,
  pdfborder={0 0 0},
}

\usepackage[capitalize,noabbrev]{cleveref}

\newcommand{\cmlabRef}[4]{%
  {\color{cmlabPrefix}#1}~#3{\color{cmlabNumber}#2}#4%
}
\newcommand{\cmlabRefParen}[4]{%
  {\color{cmlabPrefix}#1}~#3{\color{cmlabNumber}(#2)}#4%
}

\crefformat{figure}     {\cmlabRef{Fig.}{#1}{#2}{#3}}
\Crefformat{figure}     {\cmlabRef{Figure}{#1}{#2}{#3}}
\crefrangeformat{figure}%
  {{\color{cmlabPrefix}Figs.}~#3{\color{cmlabNumber}#1}#4--#5{\color{cmlabNumber}#2}#6}
\crefmultiformat{figure}%
  {\cmlabRef{Figs.}{#1}{#2}{#3}}%
  {, #2{\color{cmlabNumber}#1}#3}%
  {, #2{\color{cmlabNumber}#1}#3}%
  {, and #2{\color{cmlabNumber}#1}#3}

\crefformat{table}      {\cmlabRef{Tab.}{#1}{#2}{#3}}
\Crefformat{table}      {\cmlabRef{Table}{#1}{#2}{#3}}
\crefrangeformat{table}%
  {{\color{cmlabPrefix}Tabs.}~#3{\color{cmlabNumber}#1}#4--#5{\color{cmlabNumber}#2}#6}
\crefmultiformat{table}%
  {\cmlabRef{Tabs.}{#1}{#2}{#3}}%
  {, #2{\color{cmlabNumber}#1}#3}%
  {, #2{\color{cmlabNumber}#1}#3}%
  {, and #2{\color{cmlabNumber}#1}#3}

\crefformat{section}    {\cmlabRef{Sec.}{#1}{#2}{#3}}
\Crefformat{section}    {\cmlabRef{Section}{#1}{#2}{#3}}
\crefformat{subsection} {\cmlabRef{Sec.}{#1}{#2}{#3}}
\Crefformat{subsection} {\cmlabRef{Section}{#1}{#2}{#3}}
\crefformat{subsubsection}{\cmlabRef{Sec.}{#1}{#2}{#3}}
\Crefformat{subsubsection}{\cmlabRef{Section}{#1}{#2}{#3}}
\crefrangeformat{section}%
  {{\color{cmlabPrefix}Secs.}~#3{\color{cmlabNumber}#1}#4--#5{\color{cmlabNumber}#2}#6}
\crefmultiformat{section}%
  {\cmlabRef{Secs.}{#1}{#2}{#3}}%
  {, #2{\color{cmlabNumber}#1}#3}%
  {, #2{\color{cmlabNumber}#1}#3}%
  {, and #2{\color{cmlabNumber}#1}#3}

\crefformat{equation}   {\cmlabRefParen{Eq.}{#1}{#2}{#3}}
\Crefformat{equation}   {\cmlabRefParen{Equation}{#1}{#2}{#3}}
\crefrangeformat{equation}%
  {{\color{cmlabPrefix}Eqs.}~#3{\color{cmlabNumber}(#1)}#4--#5{\color{cmlabNumber}(#2)}#6}
\crefmultiformat{equation}%
  {\cmlabRefParen{Eqs.}{#1}{#2}{#3}}%
  {, #2{\color{cmlabNumber}(#1)}#3}%
  {, #2{\color{cmlabNumber}(#1)}#3}%
  {, and #2{\color{cmlabNumber}(#1)}#3}

\crefname{algorithm}{Algo.}{Algos.}
\Crefname{algorithm}{Algorithm}{Algorithms}
\crefformat{algorithm}  {\cmlabRef{Algo.}{#1}{#2}{#3}}
\Crefformat{algorithm}  {\cmlabRef{Algorithm}{#1}{#2}{#3}}
\crefrangeformat{algorithm}%
  {{\color{cmlabPrefix}Algos.}~#3{\color{cmlabNumber}#1}#4--#5{\color{cmlabNumber}#2}#6}
\crefmultiformat{algorithm}%
  {\cmlabRef{Algos.}{#1}{#2}{#3}}%
  {, #2{\color{cmlabNumber}#1}#3}%
  {, #2{\color{cmlabNumber}#1}#3}%
  {, and #2{\color{cmlabNumber}#1}#3}

\makeatletter
\ifx\input@path\@undefined
  \def\input@path{{arXiv/}}
\else
  \edef\input@path{{arXiv/}\input@path}
\fi
\makeatother
\usepackage[
  enable,
  labname={CMLab},
  leftlogo={assets/cornelltech_shield.png},
  leftlogowidth={9mm},
  logo={assets/cmlab_logo.png},
  logowidth={22mm}
]{cmlab_1}

